Residual Motion Splatting for Continuous Space-Time Video Super-Resolution

Continuous space-time video super-resolution produces a high-resolution, highframe-rate video from a low-resolution, low-frame-rate one at arbitrary spatial scales and temporal instants. Classical spatial multi-frame super-resolution has shown that detail beyond a single frame's sampling limit can be recovered by aligning complementary observations with sub-pixel precision and accumulating them on a finer grid. Existing learning-based methods largely depart from this principle: some align and fuse frames only at low resolution before regressing a continuous high-resolution representation, while others interpolate each frame to the output resolution before splatting. In both cases, the per-frame samples are resampled before fusion, so their sub-pixel positions are lost before frames are combined. Restoring this principle in a learned continuous model raises two challenges: estimating sub-pixel motion at unobserved times, and handling holes and occlusions when splatting a coarse grid onto a finer one. We address the first by predicting per-pixel continuous trajectories that refine linear optical-flow paths with smooth residual motion, using features integrated over the full video sequence. We address the second by directly splatting consecutive low-resolution features in a learned latent space onto a high-resolution grid at their predicted sub-pixel positions with predicted visibility weights, before a decoder resolves remaining ambiguities. This makes temporal interpolation and multi-frame superresolution a single operation. Our method improves both reconstruction fidelity and perceptual quality on multiple standard benchmarks over the state of the art, while running up to an order of magnitude faster.

==> figures/IMG_0004a/figure.tex <==
% Auto-generated by scripts/crop_figure_tool.py -- paste into your LaTeX doc.
% Requires: \usepackage{graphicx} \usepackage{xcolor} \usepackage{rotating} (or \usepackage{adjustbox})
\begin{figure*}[t]
  \centering
  \includegraphics[width=0.45\linewidth]{figures/IMG_0004a/IMG_0004a_full}
  \\ IMG\_0004a GT frame 238
  \\[4pt]
  \setlength{\fboxrule}{1.6pt}
  \setlength{\fboxsep}{0pt}
  \setlength{\tabcolsep}{2pt}
  \begin{tabular}{lccccc}
    & 234 & 236 & 238 & 240 & 242 \\
    \raisebox{\dimexpr 0.0850\linewidth+1.6pt\relax}{\raisebox{-0.5\height}{\rotatebox{90}{motif}}} & \fcolorbox[HTML]{FF9900}{FFFFFF}{\includegraphics[width=0.1533\linewidth]{figures/IMG_0004a/crops/motif/roi0/234.png}} & \fcolorbox[HTML]{FF9900}{FFFFFF}{\includegraphics[width=0.1533\linewidth]{figures/IMG_0004a/crops/motif/roi0/236.png}} & \fcolorbox[HTML]{FF9900}{FFFFFF}{\includegraphics[width=0.1533\linewidth]{figures/IMG_0004a/crops/motif/roi0/238.png}} & \fcolorbox[HTML]{FF9900}{FFFFFF}{\includegraphics[width=0.1533\linewidth]{figures/IMG_0004a/crops/motif/roi0/240.png}} & \fcolorbox[HTML]{FF9900}{FFFFFF}{\includegraphics[width=0.1533\linewidth]{figures/IMG_0004a/crops/motif/roi0/242.png}} \\
    \raisebox{\dimexpr 0.0850\linewidth+1.6pt\relax}{\raisebox{-0.5\height}{\rotatebox{90}{bfstvsr}}} & \fcolorbox[HTML]{FF9900}{FFFFFF}{\includegraphics[width=0.1533\linewidth]{figures/IMG_0004a/crops/bfstvsr/roi0/234.png}} & \fcolorbox[HTML]{FF9900}{FFFFFF}{\includegraphics[width=0.1533\linewidth]{figures/IMG_0004a/crops/bfstvsr/roi0/236.png}} & \fcolorbox[HTML]{FF9900}{FFFFFF}{\includegraphics[width=0.1533\linewidth]{figures/IMG_0004a/crops/bfstvsr/roi0/238.png}} & \fcolorbox[HTML]{FF9900}{FFFFFF}{\includegraphics[width=0.1533\linewidth]{figures/IMG_0004a/crops/bfstvsr/roi0/240.png}} & \fcolorbox[HTML]{FF9900}{FFFFFF}{\includegraphics[width=0.1533\linewidth]{figures/IMG_0004a/crops/bfstvsr/roi0/242.png}} \\
    \raisebox{\dimexpr 0.0850\linewidth+1.6pt\relax}{\raisebox{-0.5\height}{\rotatebox{90}{v3}}} & \fcolorbox[HTML]{FF9900}{FFFFFF}{\includegraphics[width=0.1533\linewidth]{figures/IMG_0004a/crops/v3/roi0/234.png}} & \fcolorbox[HTML]{FF9900}{FFFFFF}{\includegraphics[width=0.1533\linewidth]{figures/IMG_0004a/crops/v3/roi0/236.png}} & \fcolorbox[HTML]{FF9900}{FFFFFF}{\includegraphics[width=0.1533\linewidth]{figures/IMG_0004a/crops/v3/roi0/238.png}} & \fcolorbox[HTML]{FF9900}{FFFFFF}{\includegraphics[width=0.1533\linewidth]{figures/IMG_0004a/crops/v3/roi0/240.png}} & \fcolorbox[HTML]{FF9900}{FFFFFF}{\includegraphics[width=0.1533\linewidth]{figures/IMG_0004a/crops/v3/roi0/242.png}} \\
    \raisebox{\dimexpr 0.0850\linewidth+1.6pt\relax}{\raisebox{-0.5\height}{\rotatebox{90}{Ours}}} & \fcolorbox[HTML]{FF9900}{FFFFFF}{\includegraphics[width=0.1533\linewidth]{figures/IMG_0004a/crops/Ours/roi0/234.png}} & \fcolorbox[HTML]{FF9900}{FFFFFF}{\includegraphics[width=0.1533\linewidth]{figures/IMG_0004a/crops/Ours/roi0/236.png}} & \fcolorbox[HTML]{FF9900}{FFFFFF}{\includegraphics[width=0.1533\linewidth]{figures/IMG_0004a/crops/Ours/roi0/238.png}} & \fcolorbox[HTML]{FF9900}{FFFFFF}{\includegraphics[width=0.1533\linewidth]{figures/IMG_0004a/crops/Ours/roi0/240.png}} & \fcolorbox[HTML]{FF9900}{FFFFFF}{\includegraphics[width=0.1533\linewidth]{figures/IMG_0004a/crops/Ours/roi0/242.png}} \\
    \raisebox{\dimexpr 0.0850\linewidth+1.6pt\relax}{\raisebox{-0.5\height}{\rotatebox{90}{GT}}} & \fcolorbox[HTML]{FF9900}{FFFFFF}{\includegraphics[width=0.1533\linewidth]{figures/IMG_0004a/crops/GT/roi0/234.png}} & \fcolorbox[HTML]{FF9900}{FFFFFF}{\includegraphics[width=0.1533\linewidth]{figures/IMG_0004a/crops/GT/roi0/236.png}} & \fcolorbox[HTML]{FF9900}{FFFFFF}{\includegraphics[width=0.1533\linewidth]{figures/IMG_0004a/crops/GT/roi0/238.png}} & \fcolorbox[HTML]{FF9900}{FFFFFF}{\includegraphics[width=0.1533\linewidth]{figures/IMG_0004a/crops/GT/roi0/240.png}} & \fcolorbox[HTML]{FF9900}{FFFFFF}{\includegraphics[width=0.1533\linewidth]{figures/IMG_0004a/crops/GT/roi0/242.png}} \\
  \end{tabular}
  \caption{Qualitative comparison on IMG\_0004a. Full frame with ROI(s) above; enlarged crops over frames 234--242 below.}
  \label{fig:IMG_0004a}
\end{figure*}


==> figures/IMG_0004a/figure_compact.tex <==
% Generated from crop_figure_tool outputs; needs graphicx + xcolor.
\ifdefined\stcropw\else\newlength\stcropw\newlength\stcroph\newlength\stgroupw\fi
\begin{figure*}[t]
  \centering
  \begin{minipage}[c]{0.45\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/IMG_0004a/IMG_0004a_full}\par
    \vspace{2pt}{\small GT, frame 238}
  \end{minipage}\hfill
  \begin{minipage}[c]{\dimexpr0.55\linewidth-6pt\relax}
    \centering
    \setlength{\fboxrule}{0.6pt}\setlength{\fboxsep}{0pt}%
    \setlength{\stcropw}{\dimexpr(\linewidth-1.1em-6\fboxrule-0\dimexpr1pt\relax-2\dimexpr4pt\relax-2pt)/3\relax}%
    \setlength{\stcroph}{\dimexpr\stcropw*326/294\relax}%
    \ifdim\stcroph>0.09\textheight\setlength{\stcroph}{0.09\textheight}\setlength{\stcropw}{\dimexpr\stcroph*294/326\relax}\fi
    \setlength{\stgroupw}{\dimexpr1\stcropw+2\fboxrule+0\dimexpr1pt\relax\relax}%
    \def\stcrop#1#2{\fcolorbox[HTML]{#1}{FFFFFF}{\includegraphics[width=\stcropw,height=\stcroph]{#2}}}%
    \def\stlabel#1{\makebox[1.1em][l]{\rotatebox{90}{\makebox[\stcroph][c]{\small #1}}}}%
    \setlength{\baselineskip}{0pt}\setlength{\lineskip}{1.5pt}\setlength{\lineskiplimit}{0pt}%
    \makebox[1.1em]{}\makebox[\stgroupw][c]{\small $t{=}\tfrac14$}\hspace{4pt}\makebox[\stgroupw][c]{\small $t{=}\tfrac12$}\hspace{4pt}\makebox[\stgroupw][c]{\small $t{=}\tfrac34$}\par
    \stlabel{MoTIF}\stcrop{FF9900}{figures/IMG_0004a/crops/motif/roi0/236.png}\hspace{4pt}\stcrop{FF9900}{figures/IMG_0004a/crops/motif/roi0/238.png}\hspace{4pt}\stcrop{FF9900}{figures/IMG_0004a/crops/motif/roi0/240.png}\par
    \stlabel{BF-STVSR}\stcrop{FF9900}{figures/IMG_0004a/crops/bfstvsr/roi0/236.png}\hspace{4pt}\stcrop{FF9900}{figures/IMG_0004a/crops/bfstvsr/roi0/238.png}\hspace{4pt}\stcrop{FF9900}{figures/IMG_0004a/crops/bfstvsr/roi0/240.png}\par
    \stlabel{$V^3$}\stcrop{FF9900}{figures/IMG_0004a/crops/v3/roi0/236.png}\hspace{4pt}\stcrop{FF9900}{figures/IMG_0004a/crops/v3/roi0/238.png}\hspace{4pt}\stcrop{FF9900}{figures/IMG_0004a/crops/v3/roi0/240.png}\par
    \stlabel{Ours}\stcrop{FF9900}{figures/IMG_0004a/crops/Ours/roi0/236.png}\hspace{4pt}\stcrop{FF9900}{figures/IMG_0004a/crops/Ours/roi0/238.png}\hspace{4pt}\stcrop{FF9900}{figures/IMG_0004a/crops/Ours/roi0/240.png}\par
    \stlabel{GT}\stcrop{FF9900}{figures/IMG_0004a/crops/GT/roi0/236.png}\hspace{4pt}\stcrop{FF9900}{figures/IMG_0004a/crops/GT/roi0/238.png}\hspace{4pt}\stcrop{FF9900}{figures/IMG_0004a/crops/GT/roi0/240.png}\par
  \end{minipage}
\caption{Parallax on Adobe240 IMG\_0004a ($\times$4 space, $\times$8 time), at the intermediate times
between input keyframes 234 and 242. The foreground railing moves across the wall behind it, and a small
fixture on the large stairs is visible through the railing loop. Ours keeps the bar intact and the fixture
visible at every intermediate time, at the position shown in GT. $V^3$ blurs the fixture until it
almost disappears at $t{=}\tfrac12$, BF-STVSR breaks the bar where it overlaps the background, and
MoTIF smears the two layers together.}
  \label{fig:IMG_0004a}
\end{figure*}


==> figures/IMG_0012/figure.tex <==
% Auto-generated by scripts/crop_figure_tool.py -- paste into your LaTeX doc.
% Requires: \usepackage{graphicx} \usepackage{xcolor} \usepackage{rotating} (or \usepackage{adjustbox})
\begin{figure*}[t]
  \centering
  \includegraphics[width=0.45\linewidth]{figures/IMG_0012/IMG_0012_full}
  \\ IMG\_0012 GT frame 1725
  \\[4pt]
  \setlength{\fboxrule}{1.6pt}
  \setlength{\fboxsep}{0pt}
  \setlength{\tabcolsep}{2pt}
  \begin{tabular}{lccccc}
    & 1721 & 1723 & 1725 & 1727 & 1729 \\
    \raisebox{\dimexpr 0.0393\linewidth+1.6pt\relax}{\raisebox{-0.5\height}{\rotatebox{90}{motif}}} & \fcolorbox[HTML]{FF9900}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/motif/roi0/1721.png}}\hspace{1pt}\fcolorbox[HTML]{00C2C7}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/motif/roi1/1721.png}}\hspace{1pt}\fcolorbox[HTML]{E83E8C}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/motif/roi2/1721.png}} & \fcolorbox[HTML]{FF9900}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/motif/roi0/1723.png}}\hspace{1pt}\fcolorbox[HTML]{00C2C7}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/motif/roi1/1723.png}}\hspace{1pt}\fcolorbox[HTML]{E83E8C}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/motif/roi2/1723.png}} & \fcolorbox[HTML]{FF9900}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/motif/roi0/1725.png}}\hspace{1pt}\fcolorbox[HTML]{00C2C7}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/motif/roi1/1725.png}}\hspace{1pt}\fcolorbox[HTML]{E83E8C}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/motif/roi2/1725.png}} & \fcolorbox[HTML]{FF9900}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/motif/roi0/1727.png}}\hspace{1pt}\fcolorbox[HTML]{00C2C7}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/motif/roi1/1727.png}}\hspace{1pt}\fcolorbox[HTML]{E83E8C}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/motif/roi2/1727.png}} & \fcolorbox[HTML]{FF9900}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/motif/roi0/1729.png}}\hspace{1pt}\fcolorbox[HTML]{00C2C7}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/motif/roi1/1729.png}}\hspace{1pt}\fcolorbox[HTML]{E83E8C}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/motif/roi2/1729.png}} \\
    \raisebox{\dimexpr 0.0393\linewidth+1.6pt\relax}{\raisebox{-0.5\height}{\rotatebox{90}{bfstvsr}}} & \fcolorbox[HTML]{FF9900}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/bfstvsr/roi0/1721.png}}\hspace{1pt}\fcolorbox[HTML]{00C2C7}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/bfstvsr/roi1/1721.png}}\hspace{1pt}\fcolorbox[HTML]{E83E8C}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/bfstvsr/roi2/1721.png}} & \fcolorbox[HTML]{FF9900}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/bfstvsr/roi0/1723.png}}\hspace{1pt}\fcolorbox[HTML]{00C2C7}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/bfstvsr/roi1/1723.png}}\hspace{1pt}\fcolorbox[HTML]{E83E8C}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/bfstvsr/roi2/1723.png}} & \fcolorbox[HTML]{FF9900}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/bfstvsr/roi0/1725.png}}\hspace{1pt}\fcolorbox[HTML]{00C2C7}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/bfstvsr/roi1/1725.png}}\hspace{1pt}\fcolorbox[HTML]{E83E8C}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/bfstvsr/roi2/1725.png}} & \fcolorbox[HTML]{FF9900}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/bfstvsr/roi0/1727.png}}\hspace{1pt}\fcolorbox[HTML]{00C2C7}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/bfstvsr/roi1/1727.png}}\hspace{1pt}\fcolorbox[HTML]{E83E8C}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/bfstvsr/roi2/1727.png}} & \fcolorbox[HTML]{FF9900}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/bfstvsr/roi0/1729.png}}\hspace{1pt}\fcolorbox[HTML]{00C2C7}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/bfstvsr/roi1/1729.png}}\hspace{1pt}\fcolorbox[HTML]{E83E8C}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/bfstvsr/roi2/1729.png}} \\
    \raisebox{\dimexpr 0.0393\linewidth+1.6pt\relax}{\raisebox{-0.5\height}{\rotatebox{90}{v3}}} & \fcolorbox[HTML]{FF9900}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/v3/roi0/1721.png}}\hspace{1pt}\fcolorbox[HTML]{00C2C7}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/v3/roi1/1721.png}}\hspace{1pt}\fcolorbox[HTML]{E83E8C}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/v3/roi2/1721.png}} & \fcolorbox[HTML]{FF9900}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/v3/roi0/1723.png}}\hspace{1pt}\fcolorbox[HTML]{00C2C7}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/v3/roi1/1723.png}}\hspace{1pt}\fcolorbox[HTML]{E83E8C}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/v3/roi2/1723.png}} & \fcolorbox[HTML]{FF9900}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/v3/roi0/1725.png}}\hspace{1pt}\fcolorbox[HTML]{00C2C7}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/v3/roi1/1725.png}}\hspace{1pt}\fcolorbox[HTML]{E83E8C}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/v3/roi2/1725.png}} & \fcolorbox[HTML]{FF9900}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/v3/roi0/1727.png}}\hspace{1pt}\fcolorbox[HTML]{00C2C7}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/v3/roi1/1727.png}}\hspace{1pt}\fcolorbox[HTML]{E83E8C}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/v3/roi2/1727.png}} & \fcolorbox[HTML]{FF9900}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/v3/roi0/1729.png}}\hspace{1pt}\fcolorbox[HTML]{00C2C7}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/v3/roi1/1729.png}}\hspace{1pt}\fcolorbox[HTML]{E83E8C}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/v3/roi2/1729.png}} \\
    \raisebox{\dimexpr 0.0393\linewidth+1.6pt\relax}{\raisebox{-0.5\height}{\rotatebox{90}{Ours}}} & \fcolorbox[HTML]{FF9900}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/Ours/roi0/1721.png}}\hspace{1pt}\fcolorbox[HTML]{00C2C7}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/Ours/roi1/1721.png}}\hspace{1pt}\fcolorbox[HTML]{E83E8C}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/Ours/roi2/1721.png}} & \fcolorbox[HTML]{FF9900}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/Ours/roi0/1723.png}}\hspace{1pt}\fcolorbox[HTML]{00C2C7}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/Ours/roi1/1723.png}}\hspace{1pt}\fcolorbox[HTML]{E83E8C}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/Ours/roi2/1723.png}} & \fcolorbox[HTML]{FF9900}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/Ours/roi0/1725.png}}\hspace{1pt}\fcolorbox[HTML]{00C2C7}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/Ours/roi1/1725.png}}\hspace{1pt}\fcolorbox[HTML]{E83E8C}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/Ours/roi2/1725.png}} & \fcolorbox[HTML]{FF9900}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/Ours/roi0/1727.png}}\hspace{1pt}\fcolorbox[HTML]{00C2C7}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/Ours/roi1/1727.png}}\hspace{1pt}\fcolorbox[HTML]{E83E8C}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/Ours/roi2/1727.png}} & \fcolorbox[HTML]{FF9900}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/Ours/roi0/1729.png}}\hspace{1pt}\fcolorbox[HTML]{00C2C7}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/Ours/roi1/1729.png}}\hspace{1pt}\fcolorbox[HTML]{E83E8C}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/Ours/roi2/1729.png}} \\
    \raisebox{\dimexpr 0.0393\linewidth+1.6pt\relax}{\raisebox{-0.5\height}{\rotatebox{90}{GT}}} & \fcolorbox[HTML]{FF9900}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/GT/roi0/1721.png}}\hspace{1pt}\fcolorbox[HTML]{00C2C7}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/GT/roi1/1721.png}}\hspace{1pt}\fcolorbox[HTML]{E83E8C}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/GT/roi2/1721.png}} & \fcolorbox[HTML]{FF9900}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/GT/roi0/1723.png}}\hspace{1pt}\fcolorbox[HTML]{00C2C7}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/GT/roi1/1723.png}}\hspace{1pt}\fcolorbox[HTML]{E83E8C}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/GT/roi2/1723.png}} & \fcolorbox[HTML]{FF9900}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/GT/roi0/1725.png}}\hspace{1pt}\fcolorbox[HTML]{00C2C7}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/GT/roi1/1725.png}}\hspace{1pt}\fcolorbox[HTML]{E83E8C}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/GT/roi2/1725.png}} & \fcolorbox[HTML]{FF9900}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/GT/roi0/1727.png}}\hspace{1pt}\fcolorbox[HTML]{00C2C7}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/GT/roi1/1727.png}}\hspace{1pt}\fcolorbox[HTML]{E83E8C}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/GT/roi2/1727.png}} & \fcolorbox[HTML]{FF9900}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/GT/roi0/1729.png}}\hspace{1pt}\fcolorbox[HTML]{00C2C7}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/GT/roi1/1729.png}}\hspace{1pt}\fcolorbox[HTML]{E83E8C}{FFFFFF}{\includegraphics[width=0.0653\linewidth]{figures/IMG_0012/crops/GT/roi2/1729.png}} \\
  \end{tabular}
  \caption{Qualitative comparison on IMG\_0012. Full frame with ROI(s) above; enlarged crops over frames 1721--1729 below.}
  \label{fig:IMG_0012}
\end{figure*}


==> figures/IMG_0015/figure_compact.tex <==
% Generated from crop_figure_tool outputs; needs graphicx + xcolor.
\ifdefined\stcropw\else\newlength\stcropw\newlength\stcroph\newlength\stgroupw\fi
\begin{figure*}[t]
  \centering
  \begin{minipage}[c]{0.3\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/IMG_0015/IMG_0015_full}\par
    \vspace{2pt}{\small GT, frame 1568}
  \end{minipage}\hfill
  \begin{minipage}[c]{\dimexpr0.6\linewidth-6pt\relax}
    \centering
    \setlength{\fboxrule}{0.6pt}\setlength{\fboxsep}{0pt}%
    \setlength{\stcropw}{\dimexpr(\linewidth-1.1em-12\fboxrule-3\dimexpr1pt\relax-2\dimexpr4pt\relax-2pt)/6\relax}%
    \setlength{\stcroph}{\dimexpr\stcropw*390/256\relax}%
    \ifdim\stcroph>0.09\textheight\setlength{\stcroph}{0.09\textheight}\setlength{\stcropw}{\dimexpr\stcroph*256/390\relax}\fi
    \setlength{\stgroupw}{\dimexpr2\stcropw+4\fboxrule+1\dimexpr1pt\relax\relax}%
    \def\stcrop#1#2{\fcolorbox[HTML]{#1}{FFFFFF}{\includegraphics[width=\stcropw,height=\stcroph]{#2}}}%
    \def\stlabel#1{\makebox[1.1em][l]{\rotatebox{90}{\makebox[\stcroph][c]{\small #1}}}}%
    \setlength{\baselineskip}{0pt}\setlength{\lineskip}{1.5pt}\setlength{\lineskiplimit}{0pt}%
    \makebox[1.1em]{}\makebox[\stgroupw][c]{\small $\tau{=}\tfrac14$}\hspace{4pt}\makebox[\stgroupw][c]{\small $\tau{=}\tfrac12$}\hspace{4pt}\makebox[\stgroupw][c]{\small $\tau{=}\tfrac34$}\par
    \stlabel{MoTIF}\stcrop{FF9900}{figures/IMG_0015/crops/motif/roi0/1566.png}\hspace{1pt}\stcrop{00C2C7}{figures/IMG_0015/crops/motif/roi1/1566.png}\hspace{4pt}\stcrop{FF9900}{figures/IMG_0015/crops/motif/roi0/1568.png}\hspace{1pt}\stcrop{00C2C7}{figures/IMG_0015/crops/motif/roi1/1568.png}\hspace{4pt}\stcrop{FF9900}{figures/IMG_0015/crops/motif/roi0/1570.png}\hspace{1pt}\stcrop{00C2C7}{figures/IMG_0015/crops/motif/roi1/1570.png}\par
    \stlabel{BF-STVSR}\stcrop{FF9900}{figures/IMG_0015/crops/bfstvsr/roi0/1566.png}\hspace{1pt}\stcrop{00C2C7}{figures/IMG_0015/crops/bfstvsr/roi1/1566.png}\hspace{4pt}\stcrop{FF9900}{figures/IMG_0015/crops/bfstvsr/roi0/1568.png}\hspace{1pt}\stcrop{00C2C7}{figures/IMG_0015/crops/bfstvsr/roi1/1568.png}\hspace{4pt}\stcrop{FF9900}{figures/IMG_0015/crops/bfstvsr/roi0/1570.png}\hspace{1pt}\stcrop{00C2C7}{figures/IMG_0015/crops/bfstvsr/roi1/1570.png}\par
    \stlabel{$V^3$}\stcrop{FF9900}{figures/IMG_0015/crops/v3/roi0/1566.png}\hspace{1pt}\stcrop{00C2C7}{figures/IMG_0015/crops/v3/roi1/1566.png}\hspace{4pt}\stcrop{FF9900}{figures/IMG_0015/crops/v3/roi0/1568.png}\hspace{1pt}\stcrop{00C2C7}{figures/IMG_0015/crops/v3/roi1/1568.png}\hspace{4pt}\stcrop{FF9900}{figures/IMG_0015/crops/v3/roi0/1570.png}\hspace{1pt}\stcrop{00C2C7}{figures/IMG_0015/crops/v3/roi1/1570.png}\par
    \stlabel{Ours}\stcrop{FF9900}{figures/IMG_0015/crops/Ours/roi0/1566.png}\hspace{1pt}\stcrop{00C2C7}{figures/IMG_0015/crops/Ours/roi1/1566.png}\hspace{4pt}\stcrop{FF9900}{figures/IMG_0015/crops/Ours/roi0/1568.png}\hspace{1pt}\stcrop{00C2C7}{figures/IMG_0015/crops/Ours/roi1/1568.png}\hspace{4pt}\stcrop{FF9900}{figures/IMG_0015/crops/Ours/roi0/1570.png}\hspace{1pt}\stcrop{00C2C7}{figures/IMG_0015/crops/Ours/roi1/1570.png}\par
    \stlabel{GT}\stcrop{FF9900}{figures/IMG_0015/crops/GT/roi0/1566.png}\hspace{1pt}\stcrop{00C2C7}{figures/IMG_0015/crops/GT/roi1/1566.png}\hspace{4pt}\stcrop{FF9900}{figures/IMG_0015/crops/GT/roi0/1568.png}\hspace{1pt}\stcrop{00C2C7}{figures/IMG_0015/crops/GT/roi1/1568.png}\hspace{4pt}\stcrop{FF9900}{figures/IMG_0015/crops/GT/roi0/1570.png}\hspace{1pt}\stcrop{00C2C7}{figures/IMG_0015/crops/GT/roi1/1570.png}\par
  \end{minipage}
  \caption{Fast motion on Adobe240 IMG\_0015 ($\times$4 space, $\times$8 time), at the intermediate
times between input keyframes 1564 and 1572. A truck drives across the frame. Ours keeps the back of
the truck sharp and the ``LYDIG'' text on its door readable at every intermediate time. $V^3$ blurs
the truck and adds straight lines where the borders between its space-time processing blocks show
in the output, while MoTIF and BF-STVSR
produce several overlapping copies of it.}
  \label{fig:IMG_0015}
\end{figure*}

